SIC3D: Style Image Conditioned Text-to-3D Gaussian Splatting Generation

Recent progress in text-to-3D object generation enables the synthesis of detailed geometry from text input by leveraging 2D diffusion models and differentiable 3D representations. However, the approaches often suffer from limited controllability and texture ambiguity due to the limitation of the text modality. To address this, we present SIC3D, a controllable image-conditioned text-to-3D generation pipeline with 3D Gaussian Splatting (3DGS). There are two stages in SIC3D. The first stage generates the 3D object content from text with a text-to-3DGS generation model. The second stage transfers style from a reference image to the 3DGS. Within this stylization stage, we introduce a novel Variational Stylized Score Distillation (VSSD) loss to effectively capture both global and local texture patterns while mitigating conflicts between geometry and appearance. A scaling regularization is further applied to prevent the emergence of artifacts and preserve the pattern from the style image. Extensive experiments demonstrate that SIC3D enhances geometric fidelity and style adherence, outperforming prior approaches in both qualitative and quantitative evaluations.

==> sec/1_intro.tex <==
\section{Introduction}

In recent years, text-to-3D generation has advanced significantly due to pre-trained generative image diffusion models like Stable Diffusion, enabling users to create high-quality 3D assets from text descriptions without prior 3D modeling experience. Early methods mainly use Neural Radiance Fields (NeRF) to represent 3D objects, leveraging lightweight neural networks to represent complex scenes. Although NeRF allows for detailed rendering, it is computationally intensive, typically taking hours to produce a final result. To address these limitations, 3D Gaussian Splatting (3DGS) was introduced as an explicit representation format, which increases rendering efficiency by representing the scene as a set of 3D Gaussian primitives. This approach reconstructs the object's surface using multi-view images within about 10 minutes, making 3DGS a feasible solution for efficient 3D asset generation. 

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.75\linewidth]{sec/images/two-stage-diagram.pdf}
    \caption{The SIC3D pipeline consists of two stages. The \textit{Object Generation Stage} uses a text-to-3DGS generation model to obtain a base object \(O_1\) with geometry and any texture from the text input $y$. The \textit{Style Distillation Stage} distills the pattern from the style image \(I_s\) to apply on \(O_1\) producing \(O_s\).}
    \label{fig:two-stage}
\end{figure}

Despite advances in 3DGS object generation \cite{poole2022dreamfusion, tang2023dreamgaussian, yi2023gaussiandreamer}, current methods face significant challenges in achieving fine control over the generative process. These approaches rely on iterative optimization, using multi-view renderings and a pre-trained text-to-image diffusion model to ensure the 3D output aligns with input conditions. However, they require random sampling of camera viewpoints and denoise steps at each iteration, resulting in the process always producing an over-smooth result. This high degree of randomness complicates the control over generation, limiting the effectiveness and efficiency of the pipeline.

In this paper, we propose SIC3D, a novel two-stage stylized text-to-3D asset generation framework based on Gaussian Splatting. Our input takes both text and an image, where the image provides specific style information. Our two-stage process stabilizes the optimization process by decoupling the generation of geometry and the distillation of style. In the \textit{Object Generation Stage}, we introduce Variational Score Distillation (VSD) to replace Score Distillation Sampling (SDS) for 3D Gaussian Splatting generation \cite{yi2023gaussiandreamer, tang2023dreamgaussian} to address camera inconsistency and ensure general specific style appearance on the 3D object. In the \textit{Style Distillation Stage}, we further extend VSD to Variational Stylized Score Distillation (VSSD) with an IP-Adapter to incorporate the features of style images to the diffusion model of the 3D object generation via the cross-attention mechanism.
Furthermore, gradient constraint is applied to the \textit{Style Distillation Stage} to repress the emergence of artifacts.
Our experimental results show the effectiveness of the proposed method, demonstrating flexibility and robustness across various style inputs and parameter settings, allowing us to control the strength of stylization on the generated 3D objects. We make the following contributions:
\begin{itemize}
    \item We propose a novel two-stage pipeline to influence Text-to-3D Gaussian Splatting object generation with a single style image using a 2D pre-trained control model. To generate arbitrary objects with a specific style, we propose Variational Stylized Score Distillation (VSSD).
    % \item  We provide an in-depth analysis of the relationship between 3D style generation and the Classifier Free Guidance and introduce camera viewpoint processing into the style generation process.
    \item To avoid artifacts due to geometry inconsistencies when updating the 3D parameters, we propose an efficient scaling regularization term under fixed views to provide consistent stylization guidance.
    %\item We propose an efficient constraint method to control the attributes of each 3D Gaussian to avoid artifacts due to geometry inconsistencies when updating the 3D parameters.
    \item Experiments show that our method can effectively generate stylized objects, providing more potential for industry use of text-to-3D generation. Our text-image conditioned approach outperforms current SOTA 3D style transfer methods.
\end{itemize}

% In this paper, we propose SIC3D, a novel two-stage stylized text-to-3D asset generation framework based on Gaussian Splatting. 
% Our input extends beyond a simple text prompt to include an image providing specific style information. 
% Our two-stage process stabilizes the learning by decoupling the generation of geometry and the distillation of style. 
% In the geometry generation stage, we introduce Variational Score Distillation (VSD) to replace the Score Distillation Sampling (SDS) for 3D Gaussian Splatting to address camera inconsistency and ensure general specific style appearance on the 3D object. 
% In the style distillation stage, we further extend VSD to Variational Stylized Score Distillation (VSSD) with an IP-Adapter to incorporate the features of style images to the diffusion model of the 3D object generation via cross-attention mechanism.
% Furthermore, gradient constraint is applied to the \textit{Style Distillation Stage} to repress the emergence of artifacts.

% shows a promising way for generating 3D objects from multiple modalities. 
% The geometry generation stage, VSD, camera view, uncertainty
% the style distillation stage, camera projection, VSSD, IP-Adapter

% To address camera inconsistency and ensure general specific style appearance on the 3D object, we employ a camera projection layer to process camera variables 




==> sec/2_related_work.tex <==
\section{Related Work}
% add more citation
\subsection{Text-to-3D Content Generation}
The field of multi-modal content generation has achieved significant breakthroughs, particularly in text-to-image generation \cite{rombach2022high}, where models trained on large-scale text–image datasets can produce high-fidelity, high-resolution images from diverse prompts. Motivated by these successes, researchers have extended the paradigm to text-to-3D generation, which remains challenging due to the complexity of 3D object data. Early work such as DreamFields \cite{jain2022zero} employed CLIP \cite{radford2021learning} to guide NeRF optimization, while DreamFusion \cite{poole2022dreamfusion} leveraged pre-trained text-to-image diffusion models and Score Distillation Sampling (SDS) for zero-shot 3D synthesis. Building upon the SDS pipeline, subsequent work sought to improve resolution, geometry quality, and multi-view consistency. For instance, Magic3D \cite{lin2023magic3d} introduced a two-stage coarse-to-fine framework for mesh generation, MVDream \cite{shi2023mvdream} and Wonder3D \cite{long2024wonder3d} incorporated multi-view priors for NeRF-based rendering, and Zero-123 \cite{shi2023zero123++} focused on single-image-to-multi-view generation. In parallel, 3D Gaussian Splatting (3DGS) emerged as a faster alternative to NeRF, with methods such as GSGEN \cite{chen2024text}, DreamGaussian \cite{tang2023dreamgaussian}, and GaussianDreamer \cite{yi2023gaussiandreamer} achieving improved efficiency and visual quality.

Recently, research has advanced text-to-3D synthesis further by addressing issues such as the multi-face Janus problem, artifacts and limited diversity. TRELLIS \cite{trellis2024} proposes a transformer-based architecture that jointly reasons over all viewpoints, enhancing geometric coherence. ConsDreamer \cite{zhou2025consdreamer} disentangles view-conditioned guidance and enforces geometric consistency, while SegmentDreamer \cite{zhu2025segmentdreamer} introduces segmented consistency trajectory distillation to balance self- and cross-view consistency in 3DGS optimization. Dive3D \cite{bai2025dive3d} replaces SDS with Score Implicit Matching to enhance diversity without sacrificing fidelity, and GE3D \cite{li2025ge3d} reinterprets SDS as iterative 2D editing to mitigate oversmoothing. Industry has also contributed: Roblox’s Cube 3D \cite{roblox2025cube3d} tokenizes 3D shapes for text-driven mesh generation and Tencent’s Hunyuan3D-2.0 \cite{tencent2025hunyuan3d} offers low-latency, high-quality generation within seconds.

\subsection{Controllable 3D Content Generation}
To produce desired results in 3D generation pipelines, researchers have introduced additional conditioning inputs to influence the final output. Approaches like DreamBooth3D \cite{dreambooth3d}, DreamCraft3D \cite{sun2023dreamcraft3d}, HyperDreamer \cite{wu2023hyperdreamer}, and ThemeStation \cite{wang2024themestation} employ DreamBooth \cite{ruiz2023dreambooth} to fine-tune pre-trained models with existing images, generating outputs that align with the content or style of those images. ControlDreamer \cite{oh2023controldreamer} proposed utilizing Multi-View ControlNet to accept extra depth map inputs, enabling the generation of high-quality 3D content. Additionally, several methods leverage ControlNet \cite{zhang2023adding} to guide the final output with various input types, for example, YouDream \cite{mishra2024youdream} uses pose image inputs, SketchDream \cite{qu2023sketchdreamer}, Sketch3D \cite{zheng2024sketch3d}, and Control3D \cite{chen2023control3d} employ sketch inputs, and MVControl \cite{li2023mvcontrol} processes edge information.

% Our goal is to achieve efficient stylized 3DGS object generation. Dream-in-Style \cite{kompanowski2024dream} uses the attention swapping \cite{jeong2024visual} mechanism and Stylized Score Sampling loss (SSD) to alter the style of NeRF objects. StyleMe3D \cite{zhuang2025styleme3d} builds upon the SSD loss and StyleShot \cite{gao2024styleshot} to perform 3D Style Transfer on 3D objects and scenes. In contrast, our method enables the efficient and controllable generation of high-quality stylized 3D assets, effectively mitigating the Janus problem and reducing artifact formation, introducing fine-scale control to generative 3DGS.

Our goal is to achieve efficient and controllable stylization in 3D Gaussian Splatting (3DGS). Existing approaches to 3D style transfer are primarily built on NeRF or mesh-based representations. For instance, Dream-in-Style \cite{kompanowski2024dream} leverages attention swapping \cite{jeong2024visual} and Stylized Score Sampling (SSD) loss to modify NeRF objects, while StyleMe3D \cite{zhuang2025styleme3d} extends SSD loss and incorporates StyleShot \cite{gao2024styleshot} for transferring styles across 3D objects and scenes. Although these methods demonstrate the feasibility of stylizing 3D content, they often suffer from high computational cost, limited controllability, and issues such as the Janus problem. Our approach directly operates on 3DGS representations, enabling efficient generation of high-quality stylized assets with fine-grained control.

==> sec/3_methodology.tex <==
\section{Methodology}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=0.75\linewidth]{sec/images/SIC3D_v3.pdf}
    \caption{\textbf{Overview of the Style Distillation Stage.} Two pre-trained diffusion models \(\phi\), augmented with IP-Adapter, LoRA and a camera projection layer are employed to generate stylized objects \(O_s\) from the first-stage result \(O_1\), which is generated with text prompt $y$. \(I_s\) and $y$ are projected into feature space with a pre-trained CLIP model as \(e_I\) and \(e_y\). The IP-Adapter further processes the style image feature\(e_I\) and injects style pattern information into the diffusion model's cross-attention layer. Camera parameters are also projected into feature space as \(e_c\) to provide camera information to the diffusion model. Only the parameters of the 3D GS object, LoRA, and camera projection layer are trainable. \(L_{VSSD}\) and \(L_{surface}\) are used to optimize the 3D object, while \(L_{\psi}\) fine-tunes the parameters of LoRA \(\psi\) and the camera projection layer.
}
    \label{fig:sic3d}
\end{figure*}

In this section, we introduce SIC3D, our novel two-stage framework for stylized text-to-3D asset generation, which is able to distill style features from an input style image and apply this style to the 3D object (see Figure \ref{fig:two-stage}). The strong correlation between an object's style and geometry can lead to instability and inaccurate geometry if both are updated simultaneously. Iterative optimization with a pre-trained diffusion model causes layout changes that result in inconsistent texture guidance. To achieve viewpoint-consistent stylization, general geometry \(O_1\) is generated first in the \textit{Object Generation Stage}, followed by texture updates with style conditions in the \textit{Style Distillation Stage}. Section \ref{sec:stage1} describes the first stage and Section \ref{sec:stage2} describes the second stage. Section \ref{sec:discussion} discusses particular components of stage 2. 

\subsection{Stage 1: Object Generation from Text}
\label{sec:stage1}

Recent advances in 3D Gaussian Splatting (3DGS) generation \cite{yi2023gaussiandreamer, tang2023dreamgaussian, chen2024text} enable high-quality object synthesis from text. Typical pipelines initialize a coarse 3D representation—either simple primitives or shapes from pretrained 3D diffusion models \cite{nichol2022point, jun2023shap, lrm}—and iteratively refine it via guidance from a 2D diffusion model.  

Score Distillation Sampling (SDS) \cite{poole2022dreamfusion} is a commonly used optimization objective, which updates the 3D representation by taking the discrepancy between the diffusion model’s predicted noise $\hat{\epsilon}_\phi$ and the ground truth noise $\epsilon$ as the descent direction. In our work, we instead adopt Variance Score Distillation (VSD) to improve fidelity and mitigate over-smoothing:
\begin{small}
\begin{equation}
    L_{\mathrm{SDS}} = \mathbb{E}\left[ \omega(t) \, \|\hat{\epsilon}_\phi(z_t; y, t) - \epsilon\|^2 \right],
\end{equation}
\end{small}

\noindent where $z_t$ is the perturbed latent of a multi-view rendering $x = r(O,c)$ under camera $c$, $y$ is the text prompt, and $\omega(t)$ is a time-dependent weight. SDS directly updates the object parameters $O$, but suffers from noisy and inconsistent gradients, often leading to over-smoothed geometry.  

To improve fidelity, we adopt Variational Score Distillation (VSD) \cite{wang2024prolificdreamer}, which introduces a trainable Low-Rank Adaptation (LoRA) module that incorporates camera information into the guidance:
\begin{small}
\begin{equation}
    \nabla L_{\mathrm{VSD}} = \mathbb{E}\left[\omega(t)\left(\hat{\epsilon}_{\phi}(z_t; y, t) - \hat{\epsilon}_{\mathrm{LoRA}}(z_t; y, t, c)\right) \frac{\partial x}{\partial \theta} \right].
\end{equation}
\end{small}

This case-specific LoRA is optimized jointly with the 3D object, producing sharper details and more accurate geometry. In our pipeline, we use GaussianDreamer \cite{yi2023gaussiandreamer} with VSD to obtain a base object $O_1$ with correct geometry and a coarse style, serving as the input to Stage~2.  

While our main results are obtained using this VSD-based optimization pipeline, our stylization in stage 2 is not limited to a specific method to obtain the 3DGS. An alternative is to generate 3D Gaussian parameters directly with an end-to-end generation model, such as TRELLIS \cite{trellis2024} (see Supplementary Material). 
% TRELLIS \cite{trellis2024} adopts a transformer-based generator that maps text embeddings to 3DGS objects, removing the need for iterative multi-view optimization. This approach enables faster inference and potentially stronger text–geometry alignment. In this work, we primarily present results from the VSD-based method in Stage~1, while TRELLIS-based results are provided in the supplementary material for comparison.

% \subsection{Stage 1: Object Generation from Text}
% \label{sec:stage1}

% Recent advances in 3DGS generation \cite{yi2023gaussiandreamer, tang2023dreamgaussian, chen2024text} have shown its effectiveness for generating high-quality 3D objects or scenes. These methods begin by initializing Gaussian objects using either simple geometric primitives or shapes generated by pretrained 3D diffusion models \cite{nichol2022point, jun2023shap, lrm}. These initializations are then iteratively optimized until they fit the input condition. The optimization process uses a pre-trained 2D generative diffusion model to score an object's rendering, \(x\), under different camera views, which is then incorporated into a diffusion-based loss (SDS) \cite{poole2022dreamfusion} to refine the 3DGS object. Consider a rendering function \(r\). At each optimization step, a random camera variable is sampled as \(c\). With the object's parameter \(O\), we can get the rendering as \(x=r\left(O,c\right)\). The rendering will be encoded to a latent code \(z_0\) and pertubed with a random noise \(\epsilon \sim \mathcal{N}(0,I)\) for \(t\) steps. Input for the diffusion model is given as \(z_t\). The pre-trained diffusion model will predict a noise which contains the information from both the input condition and the latent code. Derived from the score matching objective \cite{kingma2024understanding}, we can obtain the following SDS loss function:
% \begin{small}
% \begin{equation}
%     min _{\mathrm{o} \in O} L_{SDS}(\mathrm{O}):=\mathbb{E}\left[\omega\left(t\right)\left(\hat{\epsilon}_{\phi}\left(z_t;y,t\right)-\epsilon\right)\right],
% \end{equation}
% \end{small}
% where \(\omega(t)\) is the weighting function, \(y\) is the text prompt, \(t\) is the sampled timestep, and \(\hat{\epsilon}_{\phi}\) is the predicted noise from the pre-trained diffusion model \(\phi\). 
% The SDS loss guides the optimization process by computing the difference between the predicted noise and the ground truth noise, thereby providing a guidance for parameter updates. The SDS loss will make the renderings obtain the information in the conditional input by updating the object. 

% In Text-to-3D generation, due to the randomness of the camera sampling strategy and the uncertainty of the model itself, there is a high level of uncertainty in the direction of the updates provided by the diffusion model to the 3D objects, which leads to an over-smooth result.
% To address this challenge, we introduce the Variational Score Distillation (VSD) \cite{wang2024prolificdreamer} loss into the \textit{Object Generation Stage} instead of SDS loss which is used in other generative 3DGS pipelines. 

% VSD loss is able to generate a high-quality result by training an additional module of learnable parameters (Low-Rank Adaption layer, LoRA). It has the ability to produce a high-fidelity object by introducing camera information into the diffusion model guidance. Its gradient form is given as:
% \begin{small}
% \begin{equation}
%     \nabla L_{VSD}:=\mathbb{E}\left[\omega\left(t\right)\left(\hat{\epsilon}_{\phi}\left(z_t;y,t\right)-\hat{\epsilon}_{LoRA}\left(z_t;y,t,c\right)\right)\frac{\partial x}{\partial \theta}\right],
% \end{equation}
% \end{small}
% where \(c\) is the camera information and \(\hat{\epsilon}_{LoRA}\) is the predicted noise from LoRA. LoRA's parameters will be trained based on the multi-view rendering, which means it's case-specific.

% In this work (see Figure \ref{fig:two-stage}), we chose to use a generative 3DGS model as the first stage (\textit{Object Generation Stage}). Specifically, we implement GaussianDreamer \cite{yi2023gaussiandreamer} and VSD loss to generate a base object \(O_1\) with correct geometry and a basic style. Both the general geometry and style of the Object Generation stage results, \(O_1\), have a high correlation with the coarse objects provided by Shap-E \cite{jun2023shap}. In the next stage (\textit{Style Distillation Stage}), the same text prompt and an additional image input are used for further generation.

\subsection{Stage 2: Style Distillation from Image}
\label{sec:stage2}

% In the second stage, we distill the features from the input style image to the first stage result, \(\mathrm{g}_1\). Specifically, we utilize a pre-trained 2D image generation control model to control the Text-to-3D generation process. 
In the second stage, we transfer features from the style image \(I_s\) to the result from the first stage, \(O_1\). To do this, we use a pre-trained 2D image control model to help guide the Text-to-3D generation.



The final results \(O_s\) align with the text prompt and style image. Style extraction from the input image is facilitated by an additional pre-trained processor, using Variational Stylized Score Distillation (VSSD) guidance to control 3D style generation. A detailed overview of the \textit{Style Distillation Stage} is given in Figure \ref{fig:sic3d}. Based on the result from the previous stage, \(O_1\), we obtain its rendering under random camera views at each step. Then, VSSD guidance is produced using both text  \(y\) and image input \(I_s\) along with the camera information \(c\) to distill the view-specific style information to the 3DGS object. After multiple steps of optimization, we get the final stylized object, \(O_s\). The following subsections introduce key components used in Stage 2 generation.
% \zxc{Mention the subsections in this section, what are their relationship to each other?}
% Different layouts on the rendering can lead to irregular patterns of change in their surfaces, causing the diffusion model to produce inconsistent guidance in terms of texture detail. In order to obtain consistent stylization results across viewpoints, it is necessary to first obtain a general geometry \(\mathrm{g}_1\) in the \textit{Geometry Generation Stage} and then update the texture using additional style conditions in the \textit{Style Distillation Stage}. The final results \(\mathrm{g}_s\) will have consistent features with text prompt and style image. To extract the style from the input image and apply it to the guidance provided by the diffusion model, we use an additional pre-trained image condition processor. We call the guidance used to control the style generation of the 3D object Variational Stylized Score Distillation (VSSD) guidance. 


\subsubsection{IP-Adapter as Image Condition Processor}
% \zxc{Which modules/models in Fig. 2 are included in 'Image Condition Processor'? What is the purpose of 'Image Condition Processor'?}
% Reorder below paragraph

To enable the diffusion model to incorporate style information from an additional image condition, we use a pre-trained IP-Adapter \cite{ye2023ip}, which acts as an Image Condition Processor. It employs a decoupled cross-attention mechanism to process both text and image inputs. The image input needs to be encoded first by the CLIP Image Encoder into a CLIP image embedding \(\mathbf{e}_I\). The information in the style image embedding is further extracted by linear projection layers of the IP-Adapter as \(\mathbf{e}'_I\). In this way the diffusion model can be influenced not just by the text embedding \(\mathbf{e}_y\), but also the specific image feature \(\mathbf{e}'_I\). 
In the \(i\)-th cross-attention layer, the feature vectors from text and image will be projected as \(K^i\) and \(V^i\), respectively. The output from the previous ResBlock and self-attention layers will be projected as \(Q^i\). The \(K^i\) and \(V^i\) from the image and text are computed respectively with \(Q^i\) and give the outputs \(\boldsymbol{Z}_{mix}^i\) for cross-attention layer \(\boldsymbol{CA}_i\). The attention values are added as the new output of the cross-attention layer. Its form of decoupled cross-attention is defined as:
\begin{small}
    \begin{equation}
    \boldsymbol{Z}_{mix}^i=\operatorname{CA}(Q^i, K_{y}^i, V_{y}^i)+\lambda \cdot \operatorname{CA}\left(Q^i, K_{I}^i, V_{I}^i\right),
\end{equation}
\end{small}

\noindent where \(\lambda\) is the hyper-parameter (IP-Adapter scale) that controls the ratio of information from text and images in the final result. Using IP-Adapter allows an image prompt to work well with a text prompt for multi-modal conditioned generation. The final results will contain features from both conditions. The IP-Adapter used in our pipeline is applied to all the cross-attention layers of the pre-trained U-Net. 

\subsubsection{Variational Stylized Score Distillation (VSSD)}

The second stage of the pipeline involves updating the surface texture through VSSD, with a pre-trained IP-Adapter integrated into the diffusion process. The primary focus is on enriching the object's surface texture, ensuring that the style features derived from the reference style image are applied consistently across multiple viewpoints.

To address camera inconsistency and apply a specific style pattern on the 3D object, we employ a camera projection layer to obtain camera embedding \(\mathbf{e}_c\). By integrating the IP-Adapter into the pre-trained diffusion model, we provide additional style information \(s\) to the diffusion model, while distilling the information of the 3D object into a LoRA module. The VSSD loss is defined as:
\begin{small}
\begin{equation}
    min _{\mathrm{o} \in O} L_{VSSD}(\mathrm{o}):=\mathbb{E}\left[\omega\left(t\right)\left(\hat{\epsilon}_{\phi}\left(z_t;y, t,s\right)-\hat{\epsilon}_{\psi}\left(z_t;y, t,c\right)\right)\right],
\end{equation}
\end{small}

\noindent and its gradient form is given as:
\begin{small}
\begin{equation}
    \nabla L_{VSSD}:=\mathbb{E}\left[\omega\left(t\right)\left(\hat{\epsilon}_{\phi}\left(z_t;y,t,s\right)-\hat{\epsilon}_{\psi}\left(z_t;y,t,c\right)\right)\frac{\partial x}{\partial \theta}\right],
\end{equation}
\end{small}

\noindent where \(\hat{\epsilon}_{\phi}(z_t;y,t,s)\) is the predicted noise from the pre-trained diffusion model \(\phi\) and IP-Adapter. 

While updating the 3D objects, the LoRA module needs to be trained at the same time. The input for the diffusion model will be the text embedding \(e_y\), camera embedding \(e_c\) and noisy latent code \(z_t\). The camera variables are provided as the camera-to-world matrix, which is projected into a camera embedding by the camera projection layer. LoRA and the camera projection layer are trained at the same time using a simple variant of diffusion loss:
\begin{small}
\begin{equation}
L_{\psi}=\mathbb{E}||\hat{\epsilon}_{\psi}\left(z_t;\varnothing,t,c\right) - \epsilon||^2.
\end{equation}
\end{small}

Note that the parameters in the camera projection layer follow those of the previous stage, but the parameters of LoRA need to be reinitialized to avoid the influence of the style learned from \(O_1\).

LoRA is able to implicitly contain information about the 3D object, enabling the model to produce geometry-consistent and style-aligned guidance across all viewpoints. VSSD loss allows the injection of style information at a controllable level, aligning the 3D object’s texture with the desired style across iterations without amplifying instability or generating artifacts. The degree of stylization from VSSD guidance depends on both the IP-Adapter scale and the sampled timestep. An ablation study of these components will be presented in the supplementary material.

% \subsubsection{Camera Sampling}
% \label{sec:discussion} 

% As proposed in NFSD \cite{nfsd}, the guidance provided by diffusion models for 3D object generation can be decomposed into two principal directions: the domain correction direction and the denoising direction. Since rendered images of 3D objects is typically out of the natural images' distribution, the denoising direction is usually noisy during each update step of the 3D Gaussian optimization. Additionally, under a random camera sampling strategy, the pseudo ground truths \cite{liang2024luciddreamer} indicated by guidance at each step become inconsistent across different views. This noisy update direction and inconsistency leads to over-smoothed surfaces and a lack of sharp details in SDS-based 3D generation. Therefore, a large classifier-free guidance (CFG) weight (e.g., 100) is typically employed to amplify the domain correction direction, or alternatively, an additional module (e.g., LoRA) \cite{wang2024prolificdreamer} may be introduced to suppress the impact of the noisy denoising direction.

% In the second stage of our pipeline, where we aim to optimize the object with a specific style, it is important to capture both low-frequency features (e.g., color distribution) and high-frequency details (e.g., patterns) from the input image. However, generation of high-frequency details are particularly sensitive to viewpoint changes and tend to become disordered when the camera viewpoints are randomly sampled (see Figure \ref{fig:ablation_camera}). To mitigate this issue and enhance the fidelity, we propose a fixed camera sampling strategy in the second stage. Specifically, we render the object from a fixed set of predefined viewpoints that collectively cover the entire surface of the object. The VSSD loss is produced based on these viewpoints. This method reduces the inconsistency in high-frequency guidance and produces texture with a detailed pattern, which leads to higher-quality stylization in the final 3D output.



\subsubsection{Scaling Constraint for 3DGS}
\label{sec:vc}

% During optimization, Gaussians may gradually grow larger to cover more pixels on the image plane, which can lead to visual artifacts and blurry stylization result.(see Figure \ref{img:vc}) To prevent this, we add a scaling constraint that keeps the influence area of each Gaussian on the image plane roughly fixed.
During optimization, Gaussians tend to expand in size to cover more pixels on the image plane. This uncontrolled growth can lead to visual artifacts and blurry stylization results (illustrated in Figure \ref{img:vc}). To address this issue, we introduce a scaling constraint that encourages each Gaussian to maintain a consistent influence area in the rendered view.

One intuitive option is to directly constrain the 3D volume of each Gaussian. However, this is not ideal, as some Gaussians may become flat in one direction while still covering a large area in the rendered view. Alternatively, constraining the number of pixels influenced by each Gaussian is more direct but leads to non-differentiable and unstable optimization.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{sec/images/volume_constraint.pdf}
    \caption{Impact of different scales of Gaussians. The red solid line indicates the target boundary, while the black dashed line represents the object surface. In the top row, where the Gaussian scale is too large, there are significant artifacts, even through the Gaussian centers are near the target boundary. This leads to a blurry boundary in the renderings. In contrast, the bottom row show that a lower level of scale leads to higher fidelity and smoother contours in the generated object.
    }
    \label{img:vc}
\end{figure}

To address this issue, we choose to regularize the approximated surface area of each Gaussian. This term is continuous and differentiable, and more accurately reflects the visible contribution of each Gaussian in image space.

We approximate the surface area of each anisotropic Gaussian using a quasi-analytical ellipsoid formula:
\begin{equation}
    A \approx 4 \pi\left(\frac{a^p b^p+a^p c^p+b^p c^p}{3}\right)^{\frac{1}{p}}, \quad \text { with } p=1.6075
\end{equation}
where $a$, $b$, $c$ denote the scaling parameters along the principal axes of each Gaussian. The constane $p$ is empirically determined \cite{thomsen1900} to minimize the approximation error of the ellipsoid surface area. 
To ensure scale uniformity across all primitives, we penalize the variance of the logarithmic surface area:

\begin{equation}
    \mathcal{L}_{\text {surface }}=\frac{1}{N} \sum_{i=1}^N\left(\log A_i-\log \bar{A}\right)^2
\end{equation}
where $A_i$ is the surface area of the i-th Gaussian and $\bar{A}$ is the mean surface area across all Gaussians. This term provides scale-invariant penalization, making the regularization robust to the overall scene scale.

% Instead of intuitively limiting the volume of each Gaussian, which could wrongly penalize flattened shapes that still cover large areas in the projection—we directly constrain their projected influence. However, we do not limit the exact number of influenced pixels, as that would be non-continuous and non-differentiable, making optimization difficult.


% By minimizing $L_{surface}$ under a fixed viewpoint setup, we encourage all Gaussians to have consistent covering regions on the renderings. This reduces view-dependent artifacts and enhances the fidelity of stylized texture transfer. The scaling constraint thus acts as a reliable prior to provide stable and consistent guidance.
By minimizing $L_{surface}$ under fixed camera viewpoints, we ensure that all Gaussians contribute evenly in the rendered images. This reduces view-dependent inconsistencies and helps produce stylized outputs with clearer textures and sharper edges. The scaling constraint thus serves as an effective prior that stabilizes training and enhances generation quality.

\subsection{Discussion}
\label{sec:discussion}

This section considers the distribution mismatch introduced by using IP-Adapter for gradient-based 3D optimization, describe how auxiliary components mitigate instability, and reflect on the broader implications for 3D stylization.

A key challenge is the distribution mismatch between standard IP-Adapter inference and our optimization setting. Normally, IP-Adapter starts from Gaussian noise and denoises toward a stylized image, whereas we feed perturbed 3D renderings into the adapter to compute gradients. This raises concerns about whether the predicted noise remains valid outside its generative trajectory. In practice, however, gradients in background regions have little effect on geometry, while object regions still receive consistent and effective style guidance. As a result, the adapter enforces stylization without introducing artifacts, which is especially important for artistic or abstract styles.

Directly applying existing 2D image style transfer methods (e.g. AdaIn \cite{huang2017arbitrary}) on rendered views tends to impose a fixed pattern across the entire image, often conflicting with the underlying object content derived from the text prompt. By contrast, using a diffusion model with IP-Adapter allows the style guidance to be integrated with the text-conditioned geometry, resolving these conflicts and producing more coherent and semantically faithful stylized 3D results.

Several additional components strengthen the overall quality and stylization. The LoRA-adapted diffusion backbone integrates viewpoint and style conditions into the predicted noise, ensuring geometry-aligned gradients across views. In addition, full-range timestep and camera sampling balance stylization strength with detail preservation. 

% Overall, our results show that IP-Adapter can be repurposed as a robust conditional guidance module for 3D stylization, decoupled from its original generative distribution. This finding opens opportunities for applying adapter-based mechanisms in broader optimization settings beyond diffusion priors.


==> sec/4_experiments.tex <==

\section{Experiments}
We compare our method quantitatively and qualitatively with one baseline method and three SOTA 3D style transfer methods: StyleGaussian \cite{liu2024stylegaussian}, G-Style \cite{kovacs2024} and SGSST \cite{galerne2024sgsst}. We also perform an ablation study for different parameters. 


\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.9\textwidth]{sec/images/teaser.pdf}
  \caption{Results from SIC3D. Objects in the left column are generated with the prompts ``An ancient Egyptian pyramid'' and ``A woven basket with a handle.'' The corresponding style images are shown in the top right of each sample.}

  \label{fig:results}
\end{figure*}

\subsection{Implementation Detail}
We follow the implementation of GaussianDreamer \cite{yi2023gaussiandreamer} and ProlificDreamer \cite{wang2024prolificdreamer} to generate a base object in the \textit{Object Generation Stage}. The ThreeStudio framework \cite{threestudio2023} is used in our experiments for stage 1 and 2 generation. All results in this section were generated using the pre-trained Stable Diffusion v1.5. In the second stage, we use a pre-trained IP-Adapter model released on huggingface: \textit{h94/IP-Adapter}, which is compatible with the Stable Diffusion v1.5 model. For camera sampling, we choose 4 fixed camera viewpoints that distribute evenly around the object with the same camera distance and elevation. 

Our experiments are performed on a single NVIDIA A100 GPU. For the first stage, the base object $O_1$ can be generated either by GaussianDreamer with VSD loss, which requires 500 optimization steps (about 5 minutes) and offers higher robustness. An alternative end-to-end model, TRELLIS, can produce \(O_1\) in about 20 seconds, but with reduced robustness; details and results for this variant are provided in the Supplementary Material. The style distillation stage takes 500 steps (approximately 5 minutes) in our experiments, chosen to ensure stability in the final output. In practice, this process typically converges after around 200 steps (about 2 minutes), with subsequent iterations giving minor refinements toward the final stylized result. During the generation process, the GPU memory usage.

% \zxc{I am expecting a subsection: Baseline Methods and Evaluation Metrics or two separated ones.}

\subsection{Comparison methods \& Evaluation Metrics}

Using the description of the style image to modify the text prompt (Stylized Prompt) serves as our baseline for generating 3D objects conditioned on both text and image. The GPT-4o model is used to image caption each style image, highlighting the style feature of the image (details are in the Supplemental Material). The extracted style description \(\hat{s}\) is added to the base text prompt \(y\) and used for generating 3D objects in a single stage. A stylized prompt is in the form \(y'=y+\text{in the style of } \hat{s}\). For example, ``a fox" and a fire image becomes ``a fox in the style of dancing flames, with bright orange and yellow fire dancing and twisting", which is used to generate a 3D object with VSD loss. (A comparison of style descriptions with different detail level is in the Supplementary Material.) 

We also evaluate SIC3D against three recent 3D style transfer methods. StyleGaussian \cite{liu2024stylegaussian} adapts the color patterns of 3D Gaussians to a 2D style image using VGG-based feature embeddings and a 3D CNN decoder, optimizing only color parameters. G-Style \cite{kovacs2024} stylizes entire 3DGS scenes by iteratively minimizing CLIP-S and NNFM losses under multi-view constraints, combined with color matching to align distributions. SGSST \cite{galerne2024sgsst} employs a multiscale SOS loss to capture global neural statistics while selectively updating only the color parameters of Gaussians for improved visual quality.

For quantitative evaluation, we adopt NNFM, RMSE, and LPIPS, following the same metrics used in prior work. In addition, we employ GPT-4o to assess the overall quality of the generated results, serving as a proxy for human evaluation as in \cite{wu2024gpt}.


\begin{figure*}[ht]
    \centering
    \hspace{1cm}
    \includegraphics[width=\linewidth]{sec/images/results_figure.pdf}
    % \caption{Comparison results for SIC3D and baseline results}
    \caption{The qualitative results for our proposed method compared with the stylized prompt baseline and state-of-the-art 3D style transfer methods (G-Style\cite{kovacs2024}, StyleGaussian\cite{liu2024stylegaussian} and SGSST\cite{galerne2024sgsst}). Each example shows three renderings from different views.}
    \label{fig:comparison}
\end{figure*}

\subsection{Qualitative Analysis}

Figure~\ref{fig:comparison} compares SIC3D with the baseline and recent SOTA methods under various text–style image input, with additional examples provided in the supplementary material. SIC3D consistently transfers stylistic patterns from the style image while preserving the underlying geometry, producing results that align more closely with the target style. Compared to the baseline stylized-prompt approach, which often introduces geometric distortions due to textual ambiguity, our two-stage strategy maintains structural integrity while achieving more significant stylization effect. Compared with StyleGaussian and G-Style, SIC3D captures accurate details from the style image and ensures visual consistency across the object surface. While SGSST enforces style consistency, it frequently generates artifacts that disrupt texture. Our method alleviates such issues through accurate style pattern preservation. Overall, SIC3D achieves a better trade-off between stylization and geometry, advancing the state of the art in stylized 3D generation.

% \subsection{Qualitative Analysis}

% We compare the final results generated by the SIC3D method with the baseline method and SOTA methods. Figure \ref{fig:comparison} shows all the generation results with different pairs of text prompts and style images. More generation results are presented in supplementary material.

% Our method demonstrates a significant improvement in stylized 3D generation, effectively applying patterns from the style image to the 3D object while maintaining accurate geometry. Visually, the generated results exhibit a compelling alignment with the target style, showcasing a notable advancement over existing approaches.

% Compared to the baseline method using a stylized prompt, our two-stage generation strategy successfully preserves the correct geometry while achieving a higher degree of stylization. Although the stylized prompt approach can generate visually appealing results, it often distorts geometry due to the ambiguity of text descriptions.

% In comparison to StyleGaussian and G-Style, our method more accurately captures and applies intricate details from the style image, ensuring both visual consistency and geometric integrity. While these methods leverage style inputs, they struggle to fully capture fine details due to the inherent limitations of text-to-image models.

% Regarding SGSST, although it introduces spatial consistency in stylization, it tends to generate artifacts that disrupt geometric integrity. Our approach mitigates such artifacts by focusing on maintaining structural accuracy while effectively transferring stylistic features.

% Overall, the proposed method establishes a new standard in stylized 3D generation, effectively balancing stylization and geometric preservation, as evidenced by the visual comparisons.


\subsection{Quantitative Analysis}

% For quantitative evaluation, we adopt three metrics to assess stylization effect. Each result is measured using CLIP-S, RMSE and LPIPS. CLIP-S computes the CLIP similarity between each generated result and the input conditions (both text and style image) using the ``clip-vit-base-patch32'' model, reflecting how well the output preserves textual content while matching the target style. NNFM (Nearest Neighbor Feature Matching) measures the degree of stylization, with lower scores indicating stronger adherence to the target style. Multi-view consistency is evaluated using LPIPS and RMSE between view-warped images. LPIPS captures perceptual differences between views, while RMSE measures pixel-level reconstruction errors, together reflecting both short-term and long-term consistency of the generated radiance fields. As shown in Table~\ref{tab:clip-s}, our method achieves a favorable balance in CLIP-S, retains low NNFM scores for enhanced stylization, and demonstrates competitive consistency performance in both LPIPS and RMSE.


For quantitative evaluation, we measure the generation results' stylization effect with three metrics: NNFM, RMSE, and LPIPS. To eliminate the influence of empty backgrounds on metrics evaluation, we apply object masks and compute all metrics only on the rendered object regions. We aim to evaluate the object under different views to obtain a fair comparison. To achieve this goal, we render each object from four fixed viewpoints and compute the three metrics for each rendering. NNFM measures style similarity using the Gram matrices of feature maps from VGG19 layers `conv1\_1', `conv2\_1', `conv3\_1', `conv4\_1', and `conv5\_1', reflecting the degree of the difference between the rendering and the style image input. Lower NNFM values indicate stronger adherence to the reference style. RMSE and LPIPS are used to assess stylization strength by comparing with the style image condition: RMSE reflects pixel-level deviations introduced by the style transfer, while LPIPS captures perceptual differences in feature space, together indicating the extent to which the generated results adhere to the target style. As shown in Table~\ref{tab:clip-s}, SIC3D demonstrates the most effective and balanced style transfer among all compared methods. In terms of NNFM, which measures style alignment, SIC3D achieves the lowest value (0.151), indicating the strongest adherence to the reference style. For RMSE, SIC3D also performs competitively (1.301), showing that stylization is applied in a controlled manner without introducing excessive pixel-level deviations. On LPIPS, SIC3D matches the performance of other approaches (0.882), suggesting that perceptual consistency is preserved despite stronger style transfer. Overall, these results highlight that SIC3D achieves effective and meaningful stylization while maintaining high perceptual plausibility.

\begin{table}[htb]
    \centering
    \footnotesize
    \begin{tabular}{@{}lcccc@{}}
    \hline
    Method & NNFM $\downarrow$ & RMSE $\downarrow$ & LPIPS $\downarrow$ \\ \hline
    % \cline{2-3}
    %        & Text Prompt & Style Image \\ \hline
    Stylized Prompt & 0.156   & 1.413 & 0.881 \\ \hline
    StyleGaussian   & 0.159   & \textbf{1.232} & 0.882 \\ \hline
    G-Style  & 0.154 & 1.390 & 0.881 \\ \hline
    SGSST  & 0.153   & 1.417 & 0.889 \\ \hline
    SIC3D  & \textbf{0.151}  & 1.301 & \textbf{0.877} \\ \hline
    \end{tabular}
    \caption{Quantitative comparison of different methods on masked renderings in terms of NNFM, RMSE, and LPIPS. Bold indicates the best performance for each metrics.}
    \label{tab:clip-s}
\end{table}

% \begin{table*}[htb]
%   \centering
%   \footnotesize
%   \begin{tabular}{@{}lcccccc@{}}
%     \toprule
%     Method & Text-asset alignment & 3D Plausibility & Text-Geometry Alignment & Texture Details & Geometry Details \\
%     \midrule
%     Stylised Prompt & 953.509 & 806.166 & 835.941 & 809.551 & 786.566 & \\
%     Stylised Prompt 2 & \textbf{1144.336} & \textbf{1076.242} & \textbf{1171.820} & \textbf{1117.779} & \textbf{1102.620} &\\
%     Textual Inversion & 850.433 & 833.166 & 812.723 & 759.995 & 795.335 & \\
%     SIC3D & 1004.874 & 962.811 & 884.226 & 943.463 & 954.461 & \\
%     \bottomrule
%   \end{tabular}
%   \caption{GPT-4o Evalutaion Results of \textit{Object Quality} (ELO score)}
%   \label{tab:comparison}
% \end{table*}

We use GPT-4o as a proxy for human evaluation to compare the performance of different methods. Following \cite{wu2024gpt}, we design a novel comparison instruction that focuses on \textit{Style Alignment} with the reference image. We also evaluate the \textit{Object Quality} of the generated objects \cite{wu2024gpt} over five aspects. Details are given in the Supplementary Material. We compare the generation results from SIC3D and other comparison methods randomly and calculate the ELO score \cite{elo1967proposed} for each method. A high ELO score suggests better performance. We randomly selected 100 combinations of 20 text prompts and 9 style images (4 realistic, 5 artistic). For each combination, 3 random seeds were selected to introduce variation. Each method was compared one-by-one for 350 times by GPT-4o with all other methods, randomly selected from all text-image-seed pairs. Evaluation results for \textit{Object Quality} and \textit{Style Alignment} can be seen in Table \ref{tab:comparison}. 

\begin{table}[htb]
  \centering
  \footnotesize
  \begin{tabular}{@{}lcc@{}}
    \toprule
    Method & Object Quality& Style Alignment \\
    \midrule
    Stylized Prompt & 1044.600 & 878.905   \\
    StyleGaussian & 925.368 & 848.153 \\
    G-Style & 1015.814 & 893.972 \\
    SGSST & 983.604 & 980.170 \\
    SIC3D & \textbf{1075.125} & \textbf{1154.929} \\
    \bottomrule
  \end{tabular}
  \caption{GPT-4o evaluation results (ELO score) for different stylized 3DGS generation methods. Bold indicates the best performance for each prompt or style. 
  }
  \label{tab:comparison}
\end{table}
% \begin{table*}[htb]
%   \centering
%   \footnotesize
%   \begin{tabular}{@{}lccccccc@{}}
%     \toprule
%     Method & Text-asset alignment & 3D Plausibility & Text-Geometry Alignment & Texture Details & Geometry Details & Style Alignment \\
%     \midrule
%     Stylised Prompt & 953.509 & 806.166 & 835.941 & 809.551 & 786.566 & 919.795& \\
%     Stylised Prompt 2 & \textbf{1144.336} & \textbf{1076.242} & \textbf{1171.820} & \textbf{1117.779} & \textbf{1102.620} & 831.920 & \\
%     Textual Inversion & 850.433 & 833.166 & 812.723 & 759.995 & 795.335 & 829.744& \\
%     SIC3D & 1004.874 & 962.811 & 884.226 & 943.463 & 954.461 & \textbf{1167.870}& \\
%     \bottomrule
%   \end{tabular}
%   \caption{GPT-4o Evalutaion Results (ELO score)}
%   \label{tab:comparison}
% \end{table*}


From the results, we can see that SIC3D has the best \textit{Style Alignment} score with the style image. For \textit{Object Quality}, SIC3D has the best generation quality, which indicates that our model can achieve 3D stylization without quality degradation under any style input. 

\subsection{Ablation study}
\label{sec:ablation}
This section demonstrates the effectiveness of our method by considering three important aspects: scaling constraint, fixed camera sampling, LoRA layers for stage 2.
% More results about the effect of IP-Adapter scale \(\lambda\) and noise scale range on the style injection will be presented in the supplementary material.

\textbf{Scaling Constraint:}
To highlight the importance of the Scaling Constraint, we conduct an ablation study focusing on the impact of the size of each Gaussian during optimization. Specifically, we vary the average scale of the Gaussians and observe how gradients propagated through pixel supervision influence the final results.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{sec/images/ablation_sc.pdf}
    \caption{Ablation study on the scaling constraint. Applying the scaling constraint in stage two (a) keeps each Gaussian’s radius small (3–4 pixels), resulting in smooth boundaries and plausible geometry. Without it (b), Gaussians expand (40–60 pixels), causing distorted geometry and artifacts due to inconsistent gradient guidance. In both images, the object's rendering appears on the left, with the normal map on the right over a grey background.}
    \label{fig:ablation}
\end{figure}

As shown in Figure \ref{fig:ablation}, larger average Gaussian scales (corresponding to Gaussians covering more pixels on the rendered images) significantly increases the occurrence of artifacts. This is because larger Gaussians aggregate gradients over broader regions, leading to inaccurate updates that deviate from fine structural details. These observations emphasize that controlling the spatial extent of Gaussians via the Scaling Constraint is crucial for reducing artifacts and ensuring high-fidelity 3D object generation.

\textbf{Camera Sampling:}
We study the effect of camera viewpoint sampling on 3D object stylization by comparing two strategies: random view sampling and fixed view sampling. As shown in Figure.~\ref{fig:ablation_camera}, the rendering pair (a) results with randomly sampled viewpoints, whereas rendering pair (b) shows results obtained from four fixed viewpoints consistently used during the \textit{Style Distillation Stage}.  


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{sec/images/ablation_camera.pdf}
    \caption{Ablation Study on Camera Sampling Strategy. (a) Random view sampling leads to lower object quality and weaker surface style patterns. (b) Fixed view sampling produces clearer geometry and more significant surface texture stylization.}
    \label{fig:ablation_camera}
\end{figure}

Random view sampling can distort dense or repetitive textures, while fixed viewpoints yield clearer and more consistent stylization across views.

% Random view sampling often introduces texture distortions, especially when the reference style contains dense or repetitive patterns. In contrast, fixed viewpoints produce more stable and faithful stylization, leading to clearer style transfer and improved consistency across views.

\textbf{LoRA layers:} We evaluate the effect of LoRA on stylized 3DGS generation in Figure ~\ref{fig:ablation_lora}. Without LoRA, surfaces are rougher and style patterns are weak. With LoRA, surfaces exhibit clear patterns closely resembling the style image, showing more faithful and consistent style transfer.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.75\linewidth]{sec/images/ablation_lora.pdf}
    \caption{Ablation Study on LoRA layer. (a) Without LoRA, the surface appears rougher and style patterns are weak. (b) With LoRA, the generated surface clearly exhibits patterns resembling those in the style image.}
    \label{fig:ablation_lora}
\end{figure}
